Combining Deep Generative Models and Multi-lingual Pretraining for Semi-supervised Document Classification

Semi-supervised learning through deep generative models and multi-lingual pretraining techniques have orchestrated tremendous success across different areas of NLP. Nonetheless, their development has happened in isolation, while the combination of both could potentially be effective for tackling task-specific labelled data shortage. To bridge this gap, we combine semi-supervised deep generative models and multi-lingual pretraining to form a pipeline for document classification task. Compared to strong supervised learning baselines, our semi-supervised classification framework is highly competitive and outperforms the state-of-the-art counterparts in low-resource settings across several languages.

==> EACL21 - Cross-Lingual Semi-Supervised Text Classification with Variational Autoencoder/01-abstract.tex <==
Semi-supervised learning through deep generative models and multi-lingual pretraining techniques have orchestrated tremendous success across different areas of NLP. Nonetheless, their development has happened in isolation, while the combination of both could potentially be effective for tackling task-specific labelled data shortage. To bridge this gap, we combine semi-supervised deep generative models and multi-lingual pretraining to form a pipeline for document classification task. Compared to strong supervised learning baselines, our semi-supervised classification framework is highly competitive and outperforms the state-of-the-art counterparts in low-resource settings across several languages.~\footnote{Code is available at \url{https://github.com/cambridgeltl/mling_sdgms}.}

==> EACL21 - Cross-Lingual Semi-Supervised Text Classification with Variational Autoencoder/02-intro.tex <==
\section{Introduction}
%One of the main challenges for modern natural language processing (NLP) models based on deep neural networks is their needs to be trained on large amounts of labelled data which is either unavailable or costly for many tasks and  languages. In line with this, 

Multi-lingual pretraining has been shown to effectively use unlabelled data through learning shared representations across languages that can be transferred to downstream tasks~\cite{DBLP:journals/tacl/ArtetxeS19,DBLP:conf/naacl/DevlinCLT19,DBLP:conf/emnlp/WuD19,DBLP:conf/nips/ConneauL19}. Nonetheless, the lack of labelled data still leads to inferior performance of the same model compared to those trained in languages with more labelled data such as English~ \cite{DBLP:conf/conll/ZemanHPPSGNP18,zhu-etal-2019-importance}. 

Semi-supervised learning is another appealing paradigm that supplements the labelled data with unlabelled data which is easy to acquire~\cite[\textit{inter alia}]{DBLP:conf/colt/BlumM98,DBLP:journals/tkde/ZhouL05,DBLP:conf/naacl/McCloskyCJ06}. In particular, deep generative models (DGMs) such as variational autoencoder (VAE; \citet{DBLP:journals/corr/KingmaW13}) are capable of capturing complex data distributions at scale with rich latent representations, and they
have been used for semi-supervised learning in various tasks in NLP~\cite{DBLP:conf/aaai/XuSDT17,DBLP:conf/acl/NeubigZYH18,DBLP:conf/acl/ChoiKL19,ijcai2019-737}, as well as inducing cross-lingual word embeddings~\cite{ijcai2017-582}, and representation learning in combination with Transformers via pretraining \citep{DBLP:journals/corr/abs-2004-04092}.

%Additionally, VAE pretraining has been proven to be effective in downstream low-resource document classifications \cite{DBLP:conf/acl/GururanganDCS19,DBLP:conf/emnlp/LiHNBY19}. The only work that we are aware of on cross-lingual VAE is \citet{ijcai2017-582}, where they achieved good cross-lingual text classification results with embeddings from a cross-lingual VAE pretrained on parallel corpus. 
%\begin{figure}[t]
%\centering
%\includegraphics[scale=1.0]{gm_2.pdf}
%\caption{Graphical models of VAE~(a), M1+M2~(b). The dashed and solid lines denotes inference and generation pass, respectively. Shaded nodes are observed, and half shaded nodes are partially observed.}
%\label{fig:graphical_models}
%\vspace{-4mm}
%\end{figure}

%To leverage the benefits of both worlds, we propose a pipeline method by combining semi-supervised DGMs (SDGMs) based on M1+M2 model %(Figure~\ref{fig:graphical_models}(a))
%~\cite{NIPS2014_5352}
%and its auxiliary (Figure~\ref{fig:graphical_models}(c)) variant~\cite{DBLP:conf/icml/MaaloeSSW16} 
%with multi-lingual pretraining under two settings: (1) where the pretraining is done using an LSTM-based VAE which can be transferred directly to SDGMs as multi-lingual encoder, and (2) where we using the pretrained mBERT model as the encoder and build and SDGM framework on top to further improve the state-of-the-art. These two designs highlights the independence of the SDGMs from the choice of the encoding architecture.\yicomment{
To leverage the benefits of both worlds, we propose a pipeline method by combining semi-supervised DGMs (SDGMs) based on M1+M2 model 
~\cite{NIPS2014_5352}
with multi-lingual pretraining. The pretrained model serves as multi-lingual encoder, and SDGMs can operate on top of it independently of encoding architecture. To highlight such independence, we experiment with two pretraining settings: (1) our LSTM-based cross-lingual VAE, and (2) the current stat-of-the-art (SOTA) multi-lingual BERT \citep{DBLP:conf/naacl/DevlinCLT19}.
%(\S\ref{sec:nxvae}).
%}

Our experiments on document classification in several languages show promising
%\yicomment{only promising}
results via the SDGM framework with different encoders, outperforming the SOTA supervised counterparts. We also illustrate that the end-to-end training of M1+M2 that was previously considered too unstable to train~\cite{DBLP:conf/icml/MaaloeSSW16} is possible with a reformulation of the objective function.

%One of the main challenges for modern natural language processing (NLP) models based on deep neural networks (DNNs) is the data scarcity problem, since an accurate DNN model 
%are generally data-hungry and 
%needs to be trained on large amounts of data which is either unavailable for many low-resource languages, or costly to obtain. 
%
%To tackle this problem, different methods have been proposed to leverage various types of data. For example, within a single model, 

%g~\cite{NIPS2014_5352,DBLP:conf/icml/MaaloeSSW16}, which have been also successfully applied to many NLP tasks





% semi-supervised learning with deepprobabilistic generative models [24,33,56], models such as variational autoencoder (VAE;[25]) with semi-supervised learning [24] are already capable of capturing effectively complex
% 3data distribution conditioned on various types of labels, outperforming other semi-supervisedmodels with smaller amount of labeled data [24,33] , which is particularly suitable forgeneral low-resource setting.However, in truly low-resource setting when the labeled, unlabeled or both types ofdata are extremely small or not even available, the monolingual signal is simply not enoughfor semi-supervised learning to perform well on the task.  For this, it is then necessary toleverage cross-lingual labeled and unlabeled data by doing cross-lingual transfer learning[13,47,3,28,42] and cross-lingual semi-supervised learning [54,18]. Given the superiorperformance, powerful model capacity and flexible model assumption of the semi-superviseddeep generative models, I conjecture that they should be expected to work also well in thecross-lingual scenario with labeled and unlabeled data from multiple languages.  Despitetheir natural fit, to the best of our knowledge, no work has ever made the effort to combinesemi-supervised deep generative models with cross-lingual data, where Wei and Deng[51]only generate cross-lingual embeddings by pretraining a VAE on parallel corpus and thendirectly apply them to downstream tasks without semi-supervised learning.The framework of semi-supervised generative model allows for easy incorporation of thecross-lingual data, so my main goal is to investigate methods to enable the model with theability of cross-lingual generalization, i.e. to perform the target task reasonably well in multi-ple languages with cross-lingual data. Furthermore, I also plan to apply more sophisticatedmodels and architectures that can model even more complex data distribution of real worldNLP, which is highly label imbalanced [53] and multi-modal [60].


%by further training on learning from unlabeled data 
%Therefore unlabeled data is also commonly used in semi-supervised to bootstrap the model by retraining on the extra data labeled by previously trained models \cite[\textit{inter alia}]{DBLP:conf/colt/BlumM98,DBLP:journals/tkde/ZhouL05,DBLP:conf/naacl/McCloskyCJ06}.
%Such problem is even more salient in low-resource setting, where 

\begin{table*}[t]
    \centering
    %\scalebox{0.50}{
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lc}
    $\mathcal{L}(\mathbf{x}, y) = \underbrace{
\mathbb{E}_{q_{\phi}(\mathbf{z}_1 | \mathbf{x})}
[
\log p_{\theta}(\mathbf{x} | \mathbf{z}_1)
]
}_\text{Reconstruction}
-
\underbrace{
\mathbb{E}_{q_{\phi}(\mathbf{z}_1 | \mathbf{x})q_{\phi}(\mathbf{z}_2 | \mathbf{z}_1, y)}
[
\log \frac{q_{\phi}(\mathbf{z}_2 | \mathbf{z}_1, y)}{p(\mathbf{z}_2)} 
+ 
\log \frac{q_{\phi}(\mathbf{z}_1 | \mathbf{x})}{p_{\theta}(\mathbf{z}_1 | \mathbf{z}_2, y)} 
]
}_\text{KL}
+
\underbrace{
\log p(y)
}_\text{Constant}
$&\multirow{2}[2]{*}[2mm]{  \includegraphics[scale=1.3]{gm_2.pdf}}\\
&\\
         $\mathcal{U}(\mathbf{x})=\underbrace{
\mathbb{E}_{q_{\phi}(\mathbf{z}_1 | \mathbf{x})}
[\log p_{\theta}(\mathbf{x} | \mathbf{z}_1)]
}_\text{Reconstruction}
-
\underbrace{
\mathbb{E}_{q_{\phi}(\mathbf{z}_1 | \mathbf{x})q_{\phi}(y | \mathbf{z}_1)q_{\phi}(\mathbf{z}_2 | \mathbf{z}_1, y)}
[\log \frac{q_{\phi}(\mathbf{z}_2 | \mathbf{z}_1, y)}{p(\mathbf{z}_2)} + 
\log \frac{q_{\phi}(\mathbf{z}_1 | \mathbf{x})}{p_{\theta}(\mathbf{z}_1 | \mathbf{z}_2, y)} +
\log \frac{q_{\phi}(y | \mathbf{z}_1)}{p(y)}
]
}_\text{KL}$&\\
    \end{tabular}}
    \vspace{-2mm}
    \caption{Labelled and unlabelled objectives for M1+M2 model (left), and its corresponding graphical model (right).}
    \label{tab:equations}
    \vspace{-2mm}
\end{table*}


==> EACL21 - Cross-Lingual Semi-Supervised Text Classification with Variational Autoencoder/04-model.tex <==
\section{SDGMs with Multi-lingual Pretraining}\label{sec:nxvae}
\paragraph{LSTM-based Encoder with VAE Pretraining.}
Our pretraining is based on the framework of \citet{ijcai2017-582}, in which they pretrain a cross-lingual VAE with parallel corpus as input. However, the parallel corpus is expensive to obtain, and only the resulting cross-lingual embeddings rather than the whole encoder could be used due to the parallel input limitation of the model. 
% In brief, each input pair of parallel sentence is processed via two language-specific BiLSTM encoders~\cite{Hochreiter:1997:LSM:1246443.1246450}, and the concatenation of the last hidden states, $h$, of the BiLSTMs is used for parametrising the posterior distribution, $q_{\phi}(\mathbf{z} | \mathbf{x}_{l1},\mathbf{x}_{l2} ) = \mathcal{N}\big(\boldsymbol{\mu}_{\phi}(\mathbf{h}), \textrm{diag}(\boldsymbol{\sigma}_{\phi}^2(\mathbf{h})\big)$. The joint semantic space across two languages showed promising qualitative results in aligning words in the cross-lingual step. However, the parallel corpus is expensive to obtain, and they only used the resulting cross-lingual embeddings while pretrained encoder was discarded. 
%\paragraph{Non-parallel Cross-lingual VAE (NXVAE).} 
To address these shortcomings, we propose non-parallel cross-lingual VAE (NXVAE),
%.
%, which allows for single non-parallel input sequence in multiple languages.
%In brief, it 
which has the same graphical model as the vanilla VAE. 
Each language $i$ is associated with its own word embedding matrix, and its input sequence $\mathbf{x}_i$ is processed via a two layer BiLSTM \citep{Hochreiter:1997:LSM:1246443.1246450} shared across languages.
We use the concatenation of the BiLSTM last hidden states as $\mathbf{h}$, and compute $q_{\phi}(\mathbf{z} | \mathbf{x}_{i})$ with Eq. \ref{eq:vae_infer}, so that $\mathbf{z}$ becomes the joint cross-lingual semantic space. 
A language specific bag-of-word decoder (BOW; \citet{pmlr-v48-miao16}) is then used to reconstruct the input sequence.
Additionally, we optimise a language discriminator as an adversary~\cite{lample2018unsupervised} to encourage the mixing of different language representations and keep the shared encoder language-agnostic. 
%Given the input sequence, the discriminator tries to maximise the probability of the correct language label whereas the encoder tries to fool the discriminator.
After pretraining NXVAE, we transfer the whole encoder, including $\boldsymbol{\mu}_{\phi}(\mathbf{h})$ and $\boldsymbol{\sigma}_{\phi}^2(\mathbf{h})$, directly into our SDGM framework and treat it as $q_{\phi}(\mathbf{z}_1 | \mathbf{x})$ component of the model (\S\ref{sec:mono}).

\paragraph{Multi-lingual BERT Encoder.} 
To show that our SDGM is effective with other encoding architectures, we use the pretrained multi-lingual BERT (mBERT; \citet{DBLP:conf/naacl/DevlinCLT19})\footnote{\url{https://github.com/google-research/bert/blob/master/multilingual.md}.} as our encoder.
Given an input sequence, the pooled \texttt{[CLS]} representation is used as $\mathbf{h}$ to compute $q_{\phi}(\mathbf{z}_1 | \mathbf{x})$~(Eq.~\ref{eq:vae_infer}).
Different from NXVAE, we initialise the parameters of $\boldsymbol{\mu}_{\phi}(\mathbf{h})$ and $\boldsymbol{\sigma}_{\phi}^2(\mathbf{h})$ randomly.


%\ehsan{ ... 2-3 sentences maximum saying we use mBERT.}
%and treat it as the $q_{\phi}(\mathbf{z}_1 | \mathbf{x})$ component of the model. Such combination is capable of taking labelled and unlabelled data from multiple languages and performing document classification in semi-supervised cross-lingual settings (\S\ref{sec:experiment}).






%Finally, we can marry the cross-lingual pretraining of NXVAE and the deep generative semi-supervised learning, so that when semi-supervised models are initialized with our NXVAE, such combination is capable of taking labeled and unlabeled data from multiple languages and performing document classification in semi-supervised cross-lingual settings (\S\ref{sec:exp_semi}).

%In doing this, we can fully leverage the powerfulness of VAE to use the cross-lingual latent variable $\mathbf{z}$ for downstream tasks in multiple languages.

%Concretely, given a sequence $\mathbf{x}_i$ from the $i$-th language out of $n$ languages, with $\mathbf{x}_i = (x_i^{1}, x_i^{2}, ... , x_i^{|\mathbf{x}_i|})$, where we denote $x_{i}^j$ the $j$-th token of the sequence in the $i$-th language, a language specific lookup embedding and a shared bi-LSTM \cite{Hochreiter:1997:LSM:1246443.1246450} followed by an MLP across languages are applied for the inference model $q_{\phi}(\mathbf{z} | \mathbf{x}_i)$:
%\begin{equation*}
%\resizebox{0.85\linewidth}{!}{
%  \begin{minipage}{\linewidth}
%\centering
%$
%\begin{aligned}
%&\mathbf{h}_i^t = \big[
%\overrightarrow{\textrm{LSTM}_{\phi}}(\mathbf{h}_i^{t-1}, \mathbf{E}_i\mathbf{x}_i^{t-1});\overleftarrow{\textrm{LSTM}_{\phi}}(\mathbf{h}_i^{t+1}, \mathbf{E}_i\mathbf{x}_i^{t+1})\big]\\
%&\mathbf{h} = \textrm{MLP}_{\phi}(\mathbf{h}_i^{|\mathbf{x}_i|}), \quad i = 1, ..., n\\
%&q_{\phi}(\mathbf{z} | \mathbf{x}_i) = \mathcal{N}\big(\mathbf{z} | \boldsymbol{\mu}_{\phi}(\mathbf{h}), \textrm{diag}(\boldsymbol{\sigma}_{\phi}^2(\mathbf{h}))\big)
%\end{aligned}
%$
%\end{minipage}
%}
%\end{equation*}
%where $\mathbf{E}_i \in \mathbb{R}^{d \times |V_i|}$ is the embedding matrix for language $i$ with dimensionality $d$ and vocabulary $V_i$, $\mathbf{x}_i^j$ is the one-hot vector of the token $x_i^j$, $\mathbf{h}_i^t$ is the concatenation of the hidden states of the forward and backward LSTMs for time step $t$, and $\boldsymbol{\mu}_{\phi}(\cdot)$ and $\boldsymbol{\sigma}_{\phi}(\cdot)$ are transformations to compute the parameters of the diagonal Gaussian posterior.
%With input from multiple languages, the deterministic $\mathbf{h}$ and stochastic $\mathbf{z}$ will encode cross-lingual information.
%During decoding, the same embedding matrix $\mathbf{E}_i$ is used to decode back input $\mathbf{x}_i$ in bag-of-word (BOW) form to avoid the KL collapse \citep{pmlr-v48-miao16} conditioned on the latent code $\mathbf{z}$:

%\begin{equation*}
%\resizebox{0.95\linewidth}{!}{
%  \begin{minipage}{\linewidth}
%\centering
%$
%\begin{aligned}
%&p_{\theta}(\mathbf{x}_i | \mathbf{z}) = \prod_{j = 1}^{|\mathbf{x}_i|}\frac{\exp{(\mathbf{z}^T\mathbf{E}_i\mathbf{x}_i^j + \mathbf{b}_i^j)}}{\sum_{k = 1}^{|V_i|}\exp{(\mathbf{z}^T\mathbf{E}_i\mathbf{x}_i^k + \mathbf{b}_i^k)}}
%\end{aligned}
%$
%\end{minipage}
%}
%\end{equation*}
%where $\mathbf{b}_i^j$ is the bias term.


%\paragraph{Adversarial training.}
%To further encourage the learning of the cross-lingual representations, we apply adversarial training by adding a language discriminator on the cross-lingual hidden state $\mathbf{h}$ after the MLP \cite{lample2018unsupervised}: 
%\begin{equation*}
%\resizebox{0.95\linewidth}{!}{
%  \begin{minipage}{\linewidth}
%\centering
%$
%\begin{aligned}
%\mathcal{J}_{dis}(\mathbf{x}_i) &= \log p(i|\mathbf{h})\\
%\mathcal{J}_{\phi}(\mathbf{x}_i) &= \log p(j|\mathbf{h}), \quad j \ne i
%\end{aligned}
%$
%\end{minipage}
%}
%\end{equation*}
%\yicomment{I try to be general in the sense that our system can handle more than 2 languages, but im not sure if the reviewer will have questions on the implementations of the adversarial equation since it's not only a two class but multi-class classification.} 


%\cleardoublepage

==> EACL21 - Cross-Lingual Semi-Supervised Text Classification with Variational Autoencoder/05-experiment.tex <==
\section{Experiments}\label{sec:experiment}
We perform document classification on the class balanced multilingual document classification corpus (MLDoc; \citet{DBLP:conf/lrec/SchwenkL18}).
Each document is assigned to one of the four news topic classes: \textit{corporate/industrial} (C), \textit{economics} (E), \textit{government/social} (G), and \textit{markets} (M).
We experiment with five representative languages: \textsc{en}, \textsc{de}, \textsc{fr}, \textsc{ru}, \textsc{zh}, and use $1\textrm{k}$ instance training set along with the standard development and test set.
For experiments with varying labelled data size, the rest training data from $1\textrm{k}$ corpus is used as unlabelled data.
The full statistics are shown in Table~\ref{tb:mldoc_info}.
Three languages (\textsc{en}, \textsc{de}, \textsc{fr}) are tested for LSTM encoder with VAE pretraining (\S\ref{sec:mono}) and all five languages for mBERT encoder (\S\ref{sec:bert}).
All documents are lowercased.
We report \textit{accuracy} for evaluation following~\citet{DBLP:conf/lrec/SchwenkL18}. 

For all experiments, We use Adam~\citep{DBLP:journals/corr/KingmaB14} as optimiser, but with different learning rates for both settings and pretraining.
We implemented the model with Pytorch\footnote{\url{https://pytorch.org/}.} 1.10~\citep{paszke2019pytorch}, and use GeForce GTX 1080Ti GPUs.
See the Appendix for details about model configurations
%, tuning 
and training.
%can be found in Appendix.

\subsection{LSTM Encoder with VAE Pretraining}\label{sec:mono}
\paragraph{Experimental Setup.} For pretraining NXVAE, we use three language pairs: \textsc{en-de}, \textsc{en-fr} and \textsc{de-fr} constructed from Europarl v7 parallel corpus \citep{Koehn2002EuroparlAM},\footnote{\url{https://www.statmt.org/europarl/}.} where only two language pairs are available:
\textsc{en}-\textsc{de} and \textsc{en}-\textsc{fr}, which consist of four datasets in total: (\textsc{en}, \textsc{de})$_{\textrm{\textsc{en}-\textsc{de}}}$, and (\textsc{en}, \textsc{fr})$_{\textrm{\textsc{en}-\textsc{fr}}}$.
For \textsc{de}-\textsc{fr}, we pair \textsc{de}$_{\textrm{\textsc{en}-\textsc{de}}}$ and \textsc{fr}$_{\textrm{\textsc{en}-\textsc{fr}}}$ directly as pseudo parallel data. 
We trim all datasets into exactly the same sentence size, and preprocess them with: tokenization, lowercasing, substituting digits with $0$, and removing all punctuations, redundant spaces and empty lines.
We randomly sample a small part of parallel sentences to build a development set.
For models which do not require parallel input, e.g. NXVAE, we mix the two datasets of a language pair together.
To avoid KL-collapse during pretraining, a weight $\alpha$ on the KL term in Eq.~\ref{eq:vae} is tuned and fixed to $0.1$~\citep{DBLP:conf/iclr/HigginsMPBGBML17,DBLP:conf/icml/AlemiPFDS018}. 
We only run one trial with fixed random seed for both pretraining and document classification. 
Training details can be found in the Appendix.


\begin{table}[t]
	\centering
    \def\arraystretch{0.95}
    {\footnotesize
	\begin{tabularx}{\columnwidth}{l XXXXX}
	\toprule
		%\multicolumn{2}{r}{}  & \multicolumn{4}{c}{Train} & \multicolumn{4}{c}{Dev} & \multicolumn{4}{c}{Test}  \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} 
		
		\multicolumn{1}{l}{} & \textsc{C} & \textsc{E} & \textsc{G} & \textsc{M} & Total\\ \toprule
		
		\multirow{3}{*}{\textsc{en}} &  
	    270 & 234 & 252 & 244 & 1000\\
	    & 228 & 238 & 266 & 268 & 1000\\
	    & 991 & 1000 & 1030 & 979 & 4000\\\cmidrule(lr){2-6}
	    
		\multirow{3}{*}{\textsc{de}} &  
		270 & 240 & 245 & 245 & 1000\\
	    & 229 & 268 & 266 & 237 & 1000\\
	    & 984 & 1026 & 1022 & 968 & 4000\\\cmidrule(lr){2-6}
	    
		\multirow{3}{*}{\textsc{fr}} &  
		227 & 262 & 258 & 253 & 1000\\
		& 257 & 237 & 237 & 269 & 1000\\
		& 999 & 973 & 998 & 1030 & 4000\\\cmidrule(lr){2-6}
		
		\multirow{3}{*}{\textsc{ru}} &  
		261 & 288 & 184 & 267 & 1000\\
		& 265 & 272 & 204 & 259 & 100\\
		& 1073 & 1121 & 706 & 1100 & 4000\\\cmidrule(lr){2-6}
		
		\multirow{3}{*}{\textsc{zh}} &  
		294 & 286 & 109 & 311 & 1000\\
		& 324 & 300 & 93 & 283 & 1000\\
		& 1169 & 1215 & 363 & 1253 & 4000\\
		
		\bottomrule       
	\end{tabularx}}%
    \vspace{-2mm}
     \caption{Statistics of MLDoc in five languages.
     Instance numbers for each class along with the total numbers are shown. 
     For each language, three rows are training, development and test set instance numbers.} \label{tb:mldoc_info}
     \vspace{-2mm}
\end{table}


%For MLDoc, we use a fixed number of labelled training data, and the rest are seen as unlabelled data. 
As our supervised baselines we compare with the following two groups:
(I) NXVAE-based supervised models which are pretrained NXVAE encoder with a multi-layer perceptron classifier on top (denoted by NXVAE-z$_1$ ($q_{\phi}(y | \mathbf{z}_1)$) or NXVAE-h ($q_{\phi}(y | \mathbf{h})$) depending on the representation fed into the classifier; or 
%models with the same architecture as 
NXVAE-z$_1$ models initialised with different pretrained embeddings: random initialisation (RAND), mono-lingual fastText (FT; \citet{Q17-1010}), unsupervised cross-lingual MUSE \cite{lample2018word}, pretrained embeddings from \citet{ijcai2017-582} (PEMB), and our resulting embeddings from pretrained NXVAE (NXEMB).\footnote{All embeddings are pretrained on the same Europarl data.} 
%We run the original code of \citet{ijcai2017-582} obtained after communicating with the authors. --- let's not include this now as it may reveal of our identity if the authors of that paper review the work.
%}
% adding a stochastic classifier $q_{\phi}(y | \mathbf{z}_1)$ or $q_{\phi}(y | \mathbf{z}_1, \mathbf{x})$ on top of NXVAE, denoted NXVAE-(X)Z, corresponding to the two semi-supervised models.
% We also experiment with the deterministic classifier $q_{\phi}(y | \mathbf{x})$ (XNVAE-X) to prove the effectiveness of the stochastic $\mathbf{z}_1$.
(II) We also pretrain a word-based BERT~(BERTW) with parameter size akin to NXVAE on the same data, and fine-tune it directly.\footnote{
%All baselines are applied in \textsc{en-de}, but only NXVAE-z$_1$ and NXVAE-h are used in the other two pairs. 
We also trained subword-based models for BERT and NXVAE, and observed similar trends. See the Appendix.}
%The second group is the state-of-the-art (SOTA) multilingual BERT \cite{DBLP:conf/naacl/DevlinCLT19}.
%\footnote{\url{github.com/google-research/bert}.}


%For our semi-supervised experiments, we initialise the encoder of SDGMs with that of the pretrained NXVAE and all other parameters including decoder randomly \citep{DBLP:conf/emnlp/LiHNBY19}.
%We set the class prior $p(y)$ as uniform distribution,
For our semi-supervised experiments, we test two types of decoders with different model capacities: BOW and GRU \cite{cho-al-emnlp14}.
We use M1+M2+BOW (GRU) to denote the model with joint training using a specific decoder, and M1+M2 to denote the original model in \citet{NIPS2014_5352} with layer-wise training.\footnote{We also compared this against a more complex Skip Deep Generative Model \citep{DBLP:conf/icml/MaaloeSSW16}, but found that end-to-end M1+M2 performs better. Details in the Appendix.} We also add a semi-supervised self-training method~\citep{DBLP:conf/naacl/McCloskyCJ06} for BERTW to leverage the unlabelled data (BERTW+ST), where we iteratively add predicted unlabelled data when the model achieves a better dev. accuracy until convergence.


\begin{table}[t]
	\centering
	{\footnotesize
    \setlength{\tabcolsep}{4.5pt}
	\begin{tabularx}{\columnwidth}{ll X}
	\toprule
		Word pair & Lang & kNNs ($k = 3$)\\\toprule
% 		\multirow{2}{*}{january (\textsc{en})}      & \textsc{en} & october, april, july\\         
% 		                                            & \textsc{de} & januar, jahres, mai\\
%         \addlinespace[0.75ex]
%         \multirow{2}{*}{januar (\textsc{de})}       & \textsc{en} & january, december, september\\ 
% 		                                            & \textsc{de} & m\"arz, dezember, juni\\\cmidrule(lr){1-3}
		                                       
		\multirow{2}{*}{president (\textsc{en})}    & \textsc{en} & mr, madam, gentlemen\\
		                                            & \textsc{de} & pr\"asident, herr, kommissar\\
		                      %                      && (president, Mr., commissioner)\\
        \addlinespace[0.75ex]
		\multirow{2}{*}{pr\"asident (\textsc{de})}  & \textsc{en} & president, mr, madam\\
		                                            & \textsc{de} & herr, kommissar, herren\\
		                      %                      && (Mr., commissioner, gentlemen)\\
		                                            \cmidrule(lr){1-3}
		                                            
		\multirow{2}{*}{great (\textsc{en})}        & \textsc{en} & deal, with, a\\
		                                            & \textsc{de} & gro{\ss}e, eine, gute\\
		                      %                      && (big, a, good)\\
        \addlinespace[0.75ex]
		\multirow{2}{*}{gro{\ss} (\textsc{de})}     & \textsc{en} & striking, gets, lucrative\\
                                                    & \textsc{de} & gering, heikel, hoch\\
                              %                      && (low, tricky, high)\\
                              \cmidrule(lr){1-3}
		                                            
		\multirow{2}{*}{said (\textsc{en})}         & \textsc{en} & already, as, been\\
		                                            & \textsc{de} & gesagt, mit, dem\\
		                      %                      && (said, with, to the)\\
        \addlinespace[0.75ex]
		\multirow{2}{*}{sagte (\textsc{de})}        & \textsc{en} & he, rightly, said\\
		                                            & \textsc{de} & vorhin, kollege, kommissar\\
		                      %                      && (earlier, colleague, commissioner)\\
		\bottomrule 
	\end{tabularx}}
    \vspace{-2mm}
    \caption{Cosine similarity-based nearest neighbours of words (left column) in embedding spaces of \textsc{en} and \textsc{de}. %calculated by cosine similarity. 
    %English glosses for German words are shown in brackets.
    } \label{tb:emb}
    \vspace{-2mm}
\end{table}



\paragraph{Qualitative Results.} 
%Examples of NXVAE learned embeddings for \textsc{en-de} are reported in Table \ref{tb:emb}, confirming 
Table \ref{tb:emb} illustrates the quality of the learned alignments in the cross-lingual space of NXVAE for \textsc{en-de} word pairs.
\paragraph{Classification Results.} 
Table~\ref{tb:semimono} (\textbf{\textsc{en-de}}) shows that within supervised models the NXVAE-z$_1$ substantially outperforms other supervised baselines with the exception of BERTW. The fact that NXVAE-z$_1$ is significantly better than NXVAE-h, suggests that pretraining has enabled $\mathbf{z}_1$ to learn more general knowledge transferable to this task.
%task-specific document level information more generalizable than the deterministic $\mathbf{h}$. 
Combining with SDGMs, our best pipeline outperforms all baselines across data sizes and languages, including BERTW+ST with bigger gaps in fewer labelled data scenario. We observe the same trend of performance in both supervised and semi-supervised DGM settings on \textbf{\textsc{en-fr}} and \textbf{\textsc{de-fr}}.

% It manifests that SDGMs powered by VAE pretraining can bootstrap the model dramatically by bringing the in-domain unlabeled data. 
For decoder, BOW outperforms the GRU, a finding in line with the results of \citet{DBLP:journals/corr/abs-1910-11856} which suggests
a few keywords seem to suffice for this task.
%without high-level understanding of the document, 
%and complex linguistic properties such as word order captured by GRU can be even disturbing. 
%where they argue that the model can just rely on a few keywords without high-level understanding of the document, and complex linguistic properties such as word order captured by GRU may be even disturbing for this task. 
The poor performance of the original M1+M2, implies the domain discrepancy between pretraining and task data, and highlights the impact of fine-tuning.
%\footnote{An analysis of behaviors of semi-supervised models to account for their performance difference in Appendix.}
In addition, our NXEMB, as a byproduct of NXVAE, performs comparably well with MUSE, and better than all other embedding models including its parallel counterpart PEMB. %which further demonstrates the advantage of our NXVAE over \citet{ijcai2017-582}.
%\footnote{We also follow \citet{NIPS2014_5352} to generate text examples conditioned on the latent variable $y$ in Appendix.}

\begin{table}[t]
	\centering
    \footnotesize
    \setlength{\tabcolsep}{2pt}
	\begin{tabularx}{\columnwidth}{@{}l cccc cccc}
	%\specialrule{.4em}{.3em}{.3em}
	\toprule
\# Labels& \textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k} &
		\textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k}\\ \toprule 
	    \textbf{\textsc{en-de}} & \multicolumn{4}{c}{\textsc{en}} & \multicolumn{4}{c}{\textsc{de}}\\ 
	    \cmidrule[1.5pt](lr){2-5}\cmidrule[1.5pt](lr){6-9}
		
		%& \textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k} &
		%\textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k}\\ \toprule 
		\textsc{nxvae}-h    & 56.5          & 61.7          & 59.5          & 78.4          & 53.6          & 66.7          & 78.9          & 87.2\\
	    \textsc{nxvae}-z$_1$    & 63.9          & 71.4          & 77.0          & 91.6          & \textbf{65.0} & 73.8          & 82.7          & 93.0\\
	    \textsc{rand}       & 50.1          & 54.2          & 62.3          & 82.5          & 47.2          & 60.8          & 69.0          & 84.8\\     
	    \textsc{ft}         & 36.3          & 49.4          & 61.1          & 80.9          & 45.0          & 54.3          & 69.2          & 86.1 \\
	    \textsc{muse}       & 59.8          &  65.4 & 71.8 & 88.4 & 45.1          & 66.2          & 79.7 & 90.4\\
	    \textsc{pemb}      & 36.4          & 53.9          & 50.9          & 84.4          & 39.4          & 52.0          & 69.0          & 86.7\\
	    \textsc{nxemb}      & 61.5 & 62.0          & 68.6          & 85.4          & 53.4 & 71.2 & 75.9          & 88.8\\
	    \cdashline{2-9}
	    	    \textsc{bertw}      & \textbf{67.7} & \textbf{72.7} & \textbf{84.6} & \textbf{91.8} & 58.1          & \textbf{77.5} & \textbf{89.2} & \textbf{94.0}\\ 
	    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
	    
	    
	    \textsc{m1+m2}      & 56.6          & 67.1          & 70.3          & -    & 52.6           & 67.2          & 76.8          & -\\
	    \textsc{m1+m2+bow}  & \textbf{79.8} & \textbf{81.7} & \textbf{87.2}          & -    & 70.5           & 79.6          & \textbf{89.7} & -\\ 
	    \textsc{m1+m2+gru}  & 75.3          & 79.4          & 84.9          & -    & \textbf{75.1}           & \textbf{80.0}          & 87.1          & -\\
	    \cdashline{2-9}
	    \textsc{bertw+st}  & 68.4 & 73.9 & 86.4 & - & 59.6 & 79.7 & 89.4 & -\\ 
	\bottomrule
	
	    \textbf{\textsc{en-fr}}& \multicolumn{4}{c}{\textsc{en}} & \multicolumn{4}{c}{\textsc{fr}}\\ 
	    \cmidrule[1.5pt](lr){2-5}\cmidrule[1.5pt](lr){6-9}
	    		%& \textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k} &
		%\textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k}\\ \toprule 
		\textsc{nxvae}-h        & \textbf{71.4} & 73.8          & 78.6          & 88.0          & 62.8          & 72.7          & 79.9          & 88.9\\
	    \textsc{nxvae}-z$_1$    & 71.2          & \textbf{75.3} & \textbf{80.4} & \textbf{91.2} & \textbf{68.3} & \textbf{75.0} & \textbf{81.4} & \textbf{91.7}\\
	    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
	    \textsc{m1+m2}      & 71.8          & 73.5          & 76.5          & -    & 66.2           & 78.7          & 79.7          & -\\
	    \textsc{m1+m2+bow}  & \textbf{81.0} & \textbf{85.5} & \textbf{88.2} & -    & 80.3           & \textbf{86.0} & \textbf{88.8} & -\\ 
	    \textsc{m1+m2+gru}  & 75.3          & 81.4          & 83.8          & -    & \textbf{80.7}  & 82.3          & 87.4          & -\\ 
	   \toprule
	   \textbf{\textsc{de-fr}} & \multicolumn{4}{c}{\textsc{de}} & \multicolumn{4}{c}{\textsc{fr}}\\ 
	    \cmidrule[1.5pt](lr){2-5}\cmidrule[1.5pt](lr){6-9}
	    		%& \textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k} &
		%\textsc{32} & \textsc{64} & \textsc{128} & \textsc{1k}\\ \toprule 
		\textsc{nxvae}-h        & 42.4          & 53.3          & 74.3          & 85.7          &  39.8   & 51.8      &    58.5    & 86.9\\
	    \textsc{nxvae}-z$_1$    & \textbf{63.3} & \textbf{75.4} & \textbf{81.3} & \textbf{92.1} & \textbf{60.1} & \textbf{71.1} & \textbf{78.4} & \textbf{91.4}\\
	    \cmidrule(lr){2-5}\cmidrule(lr){6-9}
	    \textsc{m1+m2}      & 59.1          & 70.6          & 75.4          & -    & 48.5           & 57.4          & 60.7          & -\\ 
	    \textsc{m1+m2+bow}  & \textbf{78.0} & \textbf{83.2} & \textbf{88.3}          & -    & \textbf{81.4}  & \textbf{84.5} & \textbf{88.4} & -\\ 
	    \textsc{m1+m2+gru}  & 74.6          & 80.5          & 86.2         & -    & 66.2           & 77.2          & 81.9          & -\\ 
	\bottomrule
	\end{tabularx}
    \vspace{-2mm}
     \caption{MLDoc test accuracy for \textsc{en-de}, \textsc{en-fr} and \textsc{de-fr} pairs. %The header numbers denote number of labelled training data. 
     The best results for supervised and semi-supervised models are in bold.} \label{tb:semimono}
     \vspace{-2mm}
\end{table}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.97\linewidth, trim={0.2cm 0.9cm 0.2cm 1.4cm}, clip]{result}
	 \vspace{-2mm}
	\caption{Boxplot of test accuracy scores for SUP-h and M1+M2+BOW over 5 runs. The mean is shown as white dot. The dashed line is the test mean accuracy of SUP-h trained on 1k labelled data of the corresponding language.}\label{fig:bert_result}
    \vspace{-2mm}
\end{figure*}

\subsection{Multi-lingual BERT Encoder}\label{sec:bert}
\paragraph{Experimental Setup.}
%\ehsan{(1) pretraining data for mBERT, pointing out the size of the pretrained corpus for EN vs. others. (2) tuning of the objective function, not using KL, etc. (3) instability of training and freezing.}
We use the cased mBERT, a 12 layer Transformer \citep{NIPS2017_7181} trained on Wikipedia of 104 languages with 100k shared WordPiece vocabulary.
The training corpus is larger than Europarl by orders of magnitude, and high-resource languages account for most of the corpus.
We use the best SDGM setup (M1+M2+BOW \S\ref{sec:mono}), on top of mBERT encoder against the mBERT supervised model with a linear layer as classifier (SUP-h) in 5 representative languages (\textsc{en, de, fr, ru, zh}). We report the results over 5 runs due to the training instability of BERT \citep{DBLP:journals/corr/abs-2002-06305,DBLP:journals/corr/abs-2006-04884}.
%,DBLP:journals/corr/abs-2006-04884}.

%We optimise the SDGM without the KL terms shown in Table \ref{tab:equations}, and set $\alpha = \beta$ fixed across all data sizes and languages.
\paragraph{Classification Results.}
Figure \ref{fig:bert_result} demonstrates that M1+M2+BOW outperforms the SOTA supervised mBERT (SUP-h) on average across all languages. This corroborates the effectiveness of our SDGM in leveraging unlabelled data within smaller labelled data regime, as well as its independence from encoding architecture.\footnote{Compared to smaller pretraining corpus (\S\ref{sec:mono}), we found that the representations pretrained on large corpus are less prune to overfit to the training instances of the task. We observe that training without the KL regularisation yields better performance for SDMGs+mBERT.}
As expected, the gap is generally larger with $8$ and $16$ labelled data, but reduces as the data size grows to $32$. 
The variance shows similar pattern, but with relatively large values because of the instability of mBERT.
Interestingly, the performance difference seems to be more notable in high-resource languages with more pretrained data, whereas in languages with fewer pretrained texts or vocabulary overlaps such as \textsc{ru} and \textsc{zh}, the two models achieve closer results.
%\yicomment{say something about the confidence}

==> EACL21 - Cross-Lingual Semi-Supervised Text Classification with Variational Autoencoder/06-conclusion.tex <==
\section{Conclusion}
We bridged between multi-lingual pretraining and deep generative models to form a semi-supervised learning framework for document classification.
While outperforming SOTA supervised models in several settings, we showed that the benefits of SDGMs are orthogonal to the encoding architecture or pretraining procedure.
It opens up a new avenue for SDGMs in low-resource NLP by incorporating unlabelled data potentially from different domains and languages.
Our preliminary results in cross-lingual zero-shot setting with SDGMs+NXVAE are promising, and we will continue the exploration in this direction as future work.

%but we leave its comprehensive exploration to our future work.

%We would also like to will explore the generative capacity of SDGMs for synthetic data generation to supplement the available labelled/unlabelled datasets. 
%In future, we like to investigate the regularisation effect of the KL term %for labelled/unlabelled data with 
%in the context of domain shift.
% The deep generative nature of our model allows to incorporate multi-lingual synthetic data generated by decoder in order to supplement the available labelled/unlabelled sets. 
%\ehsan{We need 1 sentence here where we finish strongly and say what the research community could accomplish/explore now that we have done this work.}.
%In future, we will utilise the generative capacity of SDGMs model by generating synthetic labelled examples. 
% The deep generative nature of our model allows to incorporate multi-lingual synthetic data generated by decoder in order to supplement the available labelled/unlabelled sets. 
% We will investigate this in our future work.
%\yicomment{after synthetic stuffs, choice of the decoder, better examples.}
%\yicomment{kl, domain adaptation, cross-lingual.}
